Humanoid Robot Co-Design: Coupling Hardware Design with Gait Generation via Hybrid Zero Dynamics

Selecting robot design parameters can be challenging since these parameters are often coupled with the performance of the controller and, therefore, the resulting capabilities of the robot. This leads to a time-consuming and often expensive process whereby one iterates between designing the robot and manually evaluating its capabilities. This is particularly challenging for bipedal robots, where it can be difficult to evaluate the behavior of the system due to the underlying nonlinear and hybrid dynamics. Thus, in an effort to streamline the design process of bipedal robots, and maximize their performance, this paper presents a systematic framework for the co-design of humanoid robots and their associated walking gaits. To this end, we leverage the framework of hybrid zero dynamic (HZD) gait generation, which gives a formal approach to the generation of dynamic walking gaits. The key novelty of this paper is to consider both virtual constraints associated with the actuators of the robot, coupled with design virtual constraints that encode the associated parameters of the robot to be designed. These virtual constraints are combined in an HZD optimization problem which simultaneously determines the design parameters while finding a stable walking gait that minimizes a given cost function. The proposed approach is demonstrated through the design of a novel humanoid robot, ADAM, wherein its thigh and shin are co-designed so as to yield energy efficient bipedal locomotion.

==> other/graveyard.tex <==
\section{Intro}

Mobile robots have become an increasingly important part of our day-to-day lives. Cars and other wheeled robots are common and offer the advantage of being incredibly energy efficient and able to move at high velocities in a stable manner compared to their walking counterparts. While walking robots have gained interest in the research communities since the 1960s, only now in recent years have they started to be used for tasks outside laboratories. Boston Dynamics have been leading the front on dynamically locomoting robots which resulted in the commercial robot SPOT Mini. Since the introduction of SPOT MINI, several other quadrupedal robots have emerged such as the MIT Mini Cheetah and the many designs based on it. The introduction of affordable dynamically stable quadrupedal robots has not only made the field more approachable, but the low cost actuators has also led to opportunities in developing low-cost humanoid robots. 

\section{HZD}

Let the configuration coordinates of some robotic system be given by $q \in \mathcal{Q} \subset \mathbb{R}^n$. Furthermore, let the full system state be given by $x = (q, \dot{q}) \in \mathcal{X} \subset \mathcal{T} \mathcal{Q}$. This leads to a second-order mechanical system which can be expressed in standard form as:

\begin{equation}
    D(q) \ddot{q} + H(q, \dot{q}) = Bu,
\end{equation}

where $D(q) \in \mathbb{R}^{n \times n}$ is the inertia matrix, $H(q, \dot{q}) \in \mathbb{R}^n$ is the drift vector, and $B \in \mathbb{R}^{n \times m}$ is the actuation matrix, and $u \in \mathcal{U} \in \mathcal{R}^m$ is the system input.

Within 

The main idea behind the HZD approach is to reduce the full-order robot system dynamics into a lower-dimensional subset of the state space that is attractive and invariant, the zero dynamics surface. This is done by defining a set of outputs that define the zero dynamics surface, and by driving these outputs to zero, stability of the closed-loop dynamics can be achieved. The outputs are often referred to as virtual constraints  because the constraints are enforced through feedback control rather than being physical constraints.

Let $y^a(q)$ be functions of the generalized coordinates which we want to control. Furthermore, let the desired function values be given by $y^d(\tau, \alpha)$, where $\tau$ is a phasing variable and $\alpha$ is a matrix of real coefficients that parameterize the desired behavior of the system. The desired outputs are often parameterized by Bezier polynomials because of their computational advantages. Using these definitions the virtual constraints can formally be defined as:

\begin{equation}
    y(q) := y^a(q) - y^d(\tau (q), \alpha),
\end{equation}

When performing periodic locomotion the robot goes through different phases depending on the behavior the robot is trying to achieve. The description of the phases and order of transitions may be described by a directed cyclic graph given by $\Gamma = \{ V, E \}$, where V is a set of vertices and E is a set of edges connecting the vertices. 

Idea is to use virtual constraints to take the full order dynamics of the system and reduce them to a lower order system without doing a model reduction. 

Walking robots goes through different phases and when impacts occur there is a jump in the states, which makes the system hybrid, which means that the hybrid dynamics must also be considered. The can be enforced through impacts maps. 

We can shape the gait based on the behavior of the robot. A point foot robot with only single support phases will have one phase, while a point foot robot with intermittent double support phases will have two phases, more complex walking which includes heel strike, double support, toe off, and single support can have four phases. During regular walking, these phases should be fixed and we can therefore setup this as constraints.

Define the zero manifold. If we can find stable periodic orbits then we can also guarantee that the full order system is stable.

\begin{equation}
    \mathcal{S} := \{(q, \dot{q}) \in \mathcal{X} \ | \ z_{nsf} = 0, \ \dot{z}_{nsf}(q, \dot{q}) < 0\}
\end{equation}

\begin{equation}
    \mathcal{D} := \{ (q, \dot{q}) \in \mathcal{X} \ | \ z_{nsf} \geq 0 \} \ \subset \mathcal{X}
\end{equation}

\subsection{Link Optimization Constraint}

\begin{figure}%
    \centering
    \subfloat[\centering Original\label{fig:holonomic_original}]{{\includegraphics[width=3cm]{figures/holonomic_original.jpg} }}%
    \qquad
    \subfloat[\centering Extended\label{fig:holonomic_extended}]{{\includegraphics[width=3cm]{figures/holonomic_extended.jpg} }}%
    \caption{Visualization of an extended link.}%
    \label{fig:holonomic_contraints}%
\end{figure}

To be able to also optimize over robot dimensions in the HZD gait optimization loop we need to add another set of constraints. Consider the case where we have a kinematic model with a link $\alpha_i$ which we want to find the optimal value of, as shown in Fig. \ref{fig:holonomic_original}. The first step is to extend the robot model by adding an additional degree of freedom $\tilde{\theta}_i$ in the form of a prismatic joint after $\alpha_i$. The new variable $\tilde{\theta}_i$ is used to connect $\alpha_i$ to $\tilde{\alpha}_i$, which is a massless link. 

In most cases the joint $\tilde{\theta}_i$ will be allowed to vary between some minimum and maximum value which makes it necessary to lower and upper bound the virtual joint depending on the minimum and maximum allowable length of $\alpha_i$. Furthermore, it is important to note that since $\tilde{\theta}_i$ will be fixed on the actual robot it may not change throughout the gait, meaning that the velocity of holonomic constraint must be kept equal to zero, i.e. $\dot{\tilde{\theta}}_i = 0$.

For each link we want to optimize over the constraints specified above must be satisfied. Combing this with constraints specified in xxx, xxx, xxx, and xxx, results in the following optimization problem.

\begin{equation}
    \begin{split}
        \{\alpha^*, X^*\} = \underset{\alpha, X}{argmin} & \ \Phi(X) \\
        s.t. \quad & \dot{x} = f_{cl}(x) \\
        & \Delta(\mathcal{S} \And \mathcal{Z}_\alpha) \subset \mathcal{Z}_\alpha \\
        & X_{min} \leq X \leq X_{max} \\
        & \tilde{\theta}_{min} \leq \tilde{\theta} \leq \tilde{\theta}_{max} \\
        & \dot{\tilde{\theta}} = 0
    \end{split}
    \label{eq:optimization_problem}
\end{equation}

\newpage

Whereas the constraints in xxx, xxx, and xxx can be used to ensure stable periodic walking, the cons

Optimization over link dimensions and relative orientations 

Want to optimize dimensions, this can be to find link lengths or to find the angle between two fixed links.

We normally want to optimize over the variable over some prespecified domain, add constraints for lower bound and upper bounds. 

To add the constraint to the optimization problem we to enforce that the extended joint is fixed throughout the duration of the gait, that is, we need to set the velocity to zero. This is shown through setting the upper bound and lower bound.

To include the ability to optimize over link lengths for a symmetric robot, it is also necessary to add a constraint ensuring that the extendable joint is equal, or a mirror to its counterpart depending on the need. 


\newpage

\subsection{Co-Design HZD Loop}

URDFs are generated automatically based on two parameters.

To do this it was necessary to make the inertial properties as functions of the link lengths. Make plots showing how the change together. 

\begin{algorithm}
\caption{HZD Co-Design Algorithm}\label{alg:co_design_hzd}
\begin{algorithmic}
\State {$D_t = [{t_{min}:\Delta_t:{t_{max}}}] \in \mathbb{R}^N$}
\State {$D_s = [{s_{min}:\Delta_s:{s_{max}}}] \in \mathbb{R}^M$}
\For{$n = 1$ to $N$}                    
    \For{$m = 1$ to $M$}                    
        \State {$\alpha_{t, 0} = D_{t}(i)$}
        \State {$\alpha_{s, 0} = D_{s}(j)$}
        \State {$k = 0$}
        \While{$|\alpha_{t, k} - \alpha_{t, k-1}| + |\alpha_{s, k} - \alpha_{s, k-1}| > \Delta$} 
            \State {$k = k + 1$}
            \State {$model = GenerateModel(\alpha_{t, k-1}, \alpha_{s, k-1})$}
            \State {$[\alpha_{t, k}, \alpha_{s, k}] = Solve(NLP, model)$}
        \EndWhile
        \State {$\alpha^{i, j}_{t, final} = \alpha_{t, k}$}
        \State {$\alpha^{i, j}_{s, final} = \alpha_{s, k}$}
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

==> other/hzd_old.tex <==
\section{HZD GAIT GENERATION}

A robot performing locomotion goes through multiple continuous phases separated by discrete impacts. The mix of continuous and discrete dynamics makes the system hybrid. To control such systems, HZD control has proven itself to be a powerful tool. In this section, we present the HZD framework and how it can be used together with trajectory optimization to produce stable walking trajectories for the closed-loop system. 

\subsection{Hybrid Zero Dynamics Framework}

Let the configuration coordinates of some robotic system be given by $q \in \mathcal{Q} \subset \mathbb{R}^n$. Furthermore, let the full system state be given by $x = (q, \dot{q}) \in \mathcal{X} \subset \mathcal{T} \mathcal{Q}$. This leads to a second-order mechanical system which can be expressed in standard form as:
\begin{equation}
    D(q) \ddot{q} + H(q, \dot{q}) = Bu,
\end{equation}

where $D(q) \in \mathbb{R}^{n \times n}$ is the inertia matrix, $H(q, \dot{q}) \in \mathbb{R}^n$ is the drift vector, $B \in \mathbb{R}^{n \times m}$ is the actuation matrix, and $u \in \mathcal{U} \in \mathcal{R}^m$ is the system input.

\todo[inline]{Write about HZD multi-domain systems.}

\todo[inline]{
In this HZD explanation, we only consider the case when we have two domains, defined by whichever foot is the stance foot and which is the swing foot. Let the swing foot height above the ground be defined as $z_{nsf} : \mathcal{Q} \rightarrow \mathbb{R}$. We then have that the set of admissible states within the domain are given by:
\begin{equation}
    \mathcal{D} := \{ (q, \dot{q}) \in \mathcal{X} \ | \ z_{nsf} \geq 0 \} \ \subset \mathcal{X}
\end{equation}
The impact of the swing foot with the ground denotes the edge which triggers the transition from one domain to another. The region in which this occurs is denoted as the switching surface $\mathcal{S} \subset \mathcal{D}$ which is defined as:
\begin{equation}
    \mathcal{S} := \{(q, \dot{q}) \in \mathcal{X} \ | \ z_{nsf} = 0, \ \dot{z}_{nsf}(q, \dot{q}) < 0\}
\end{equation}
The impact of the swing foot with the ground leads to a discrete change in the states and this change can be captured by using a reset map $\Delta : \mathcal{S} \rightarrow \mathcal{X}$, which can be defined as:
}
\begin{equation}
    x^+ = \Delta(x^-), \quad x^- \in \mathcal{S}
    \label{eq:reset_map}
\end{equation}
where $x^-$ and $x^+$ refer to the pre- and post-impact states respectively. 

By combining the continuous dynamics within a domain and the reset map from \ref{eq:reset_map}, the single-domain hybrid control system is obtained:
\begin{equation}
    \mathcal{HC} = 
    \begin{cases}
        \dot{x} = f_v(x) + g_v(x)u \quad & x\notin \mathcal{S}_v \\
        x^+ = \Delta(x^-) & x^- \in \mathcal{S}_v
    \end{cases}
\end{equation}

Adding all the different domains leads to the multi-domain hybrid dynamical system given by:
\begin{equation}
    \mathcal{HC} = (\Gamma, \mathcal{D}, \mathcal{U}, \mathcal{S}, \Delta, FG)   
    \label{eq:hzd_system}
\end{equation}
The idea behind the HZD framework is to reduce the hybrid dynamical system in \ref{eq:hzd_system} into a lower dimensional system. Let the set of outputs that we want to control be given by $y^a(q)$, and let the desired outputs be given by $y^d(\tau(q), \alpha)$. Furthermore, we define the outputs $y : \mathcal{Q} \rightarrow \mathbb{R}^m$ as the difference between the two, i.e.:
\begin{equation}
    y(q) := y^a(q) - y^d(\tau (q), \alpha),
    \label{eq:output_constraint}
\end{equation}
When the outputs and their derivatives are equal to zero, we say that the residual dynamics revolve on the zero dynamics surface which is defined as:
\begin{equation}
    \mathcal{Z}_{\alpha} := \{ x \in \mathcal{D} \ | \ y(q, \alpha) = 0, \ \dot{y}(q, \alpha) = 0 \}
    \label{eq:zero_dynamics_surface}
\end{equation}
In \ref{eq:output_constraint}, the desired outputs are parameterized by $\tau(q)$ which is a phasing variable and $\alpha$ which is a collection of Bézier coefficients. By using a feedback controller $u(x)$ we can drive $y$ to zero exponentially which leads to exponential convergence to the zero dynamics surface on the continuous dynamics. Furthermore, to ensure stability of the hybrid system as a whole, we must ensure that the reset map maps the post-impact state onto the zero dynamics surface. This HZD condition can be enforced through the following condition:
\begin{equation}
    \Delta (\mathcal{S} \cap \mathcal{Z}_\alpha) \in \mathcal{Z}_\alpha
\end{equation}

==> other/results_original.tex <==
\section{Humanoid Co-Design Optimization Results}

The humanoid co-design optimization problem was run from a large variety of initial thigh and shin lengths. 

The setup in \ref{sec:adam_co-design} together with the parameters in Tab. \ref{tab:gait_constraints} was 

In this section we analyze the results obtained after running the algorithm presented in \ref{sec:co_design_framework}. The algorithm was ran for 441 different initial conditions where the initial thigh and shin lengths were uniformly distributed in a 2D grid between the minimum and maximum values from Tab. \ref{tab:gait_constraints}. 

Fig. \ref{fig:convergence_of_lengths} visualizes how the link lengths converge very closely to the same values irrespective of their initial values. In Tab. \ref{tab:optimization_results} several of the key parameters from the optimization is presented. From the table it can be seen that the optimal thigh length of $0.25 m$ is slightly shorter than the optimal shin length of $0.26 m$. Both variables converged with a very high accuracy where the standard deviation (std) is below $1.5e-3$ for both.  

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/converged_lengths.eps}
    \caption{A figure how the link lengths and thigh lengths converge from their initial values when using Co-Design-HZD algorithm.}
    \label{fig:convergence_of_lengths}
\end{figure}

\begin{table}
\caption{A table showing the average of and mean for the converged gaits after running from 25 different initial link length combinations.}
\label{tab:optimization_results}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Parameter & Mean Limit & Std \\
\hline
Thigh Length & $0.2477 [m]$ & $0.7e-3 [m]$ \\
\hline
Shin Length & $0.2590 [m]$ & $1.5e-3 [m]$ \\
\hline
Step Length & $0.2936 [m]$ & $0.0261 [m]$ \\
\hline
Step Duration & $0.8570 [s]$ & $0.90296 [s]$ \\
\hline
Walking Speed & $0.3420 [m/s]$ & $0.0196 [m/s]$ \\
\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Computational Cost}

The entire optimization loop took approximately 20 hours to run, where the run time scales linearly, O(n) with the number of samples. For the experiment ran here we chose to use a large number of samples to demonstrate consistency of the method across a wide range of initial conditions. In general, when applying the method to a specific hybrid zero system, you could get away with a significantly lower number of samples. Figure xxx shows how the design variables converge very fast, even with only a few samples. 

The most time consuming part of each sample optimization is the generation of the mex files used in FROST. These account for about XXX percent of the time, so an optimization tool not using this is likely to be able to speed up the process significantly. The time to generate the mex files scales quadratically $O(n^2)$ with the number of DoFs, therefore it can be wise to remove irrelevant DoFs when performing the optimization loop.

% Talk about how reasonable the results are by comparing it to a human of similar diemsions. 

% Add point in the table on how many iterations that were necessary to get convergence in each case. Explain how the link lengths often converge very fast to their near final values and that the values do not change too much after updating the model, which makes sense as the inertial changes are not drastic. 

==> other/xx_method.tex <==
\section{Application of the Co-Design Framework to (NAME)}\label{sec:adam_co-design}
\blue{Specific considerations for humanoid}

\subsection{Augmenting the Robot Model}
The main idea of the Co-Design HZD Algorithm is to provide a way to choose mechanical design dimensions such as link length by using HZD gait generation in the design loop to optimize some cost function. The method assumes that a mechanical design is already made and that it is possible to change the design variables in the CAD model to update the robot model. For this paper, the two parameters we chose to optimize over were the thigh lengths and shin lengths of a 20 DoF humanoid robot, with 3 DoFs in each arm, and 4 DoFs in each leg, as shown in Fig. \ref{fig:humanoid_dofs_original}. To make it possible to optimize over the link lengths we make an \blue{extended} robot model, where we add prismatic joints to the thighs and shins as shown in Fig \ref{fig:humanoid_dofs_extended}. This effectively scales the robot into a 22 DoF system. In the extended robot model we make the four prismatic links massless so that the link length inertias are still defined around their original locations. In the Co-Design-HZD algorithm we deal with handling how the leg links inertia's changes with the lengths.

\begin{figure}%
    \centering
    \subfloat[\centering Original\label{fig:humanoid_dofs_original}]{{\includegraphics[width=3cm]{figures/humanoid_original.jpg} }}%
    \qquad
    \subfloat[\centering Extended\label{fig:humanoid_dofs_extended}]{{\includegraphics[width=3cm]{figures/humanoid_extended.jpg} }}%
    \caption{The humanoid's original and the extended configuration space needed to perform the Co-Design-HZD Algorithm.}%
    \label{fig:humanoid_dofs}%
\end{figure}

\subsection{HZD Co-Design Algorithm}

Even though solving the extended optimization problem in \ref{eq:extended_optimization_problem} can be used to obtain the optimal link lengths while finding the optimal gait, it does not account for fact that changing the link lengths will ultimately also affect the inertial properties of the extendable joints. A shorter joint  


\subsection{Automatic Robot Model Generation}\label{sec:model_generation}
To solve the optimization problem outlined in section \ref{sec:frost_setup} it is necessary to provide FROST with a Unified Robot Description Format (URDF) model, which is an XML formatted file containing a complete description of the robot's kinematic and inertial properties. Because the algorithm in \ref{alg:co_design_hzd} requires the user to provide an accurate robot model for arbitrary thigh and shin lengths within their respective bounds, it was necessary to automate the model generation process. To achieve this a function $GenerateModel(thigh\_length, shin\_length)$ was created, where the two input arguments are the thigh lengths and the shin lengths, and based on this a robot model is generated. 

Since the inertial properties of the links depend on their lengths, it was necessary to obtain a function relating each of the nine inertial properties listed in table \ref{tab:inertial_values} to the link lengths. For simple geometric shapes, this can be done exactly, but as each of the links have very complex geometry such calculations were intractable. To circumvent this we employed an empiric approach where we uniformly extracted the inertial properties for 10 different thigh and shin lengths, and then used 3rd-order polynomials to fit the data. Despite the small number of inertial property samples, we were able to fit the polynomials with near-perfect accuracy as table \ref{tab:inertial_values} shows. In general, a polynomial of this order should be able to estimate the inertial properties of most links with high accuracy because of the nature of inertial properties.

\begin{table}
\caption{The average percent-wise errors between the true and approximated inertial values at the sample points.}
\label{tab:inertial_values}
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|}
\hline
Link & $x_c$ & $y_c$ & $z_c$ & $I_{xx}$ & $I_{yy}$ & $I_{zz}$ & $I_{xy}$ & $I_{xz}$ & $I_{yz}$ \\  
\hline
Thigh & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 \\
\hline
Shin & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 \\
\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Co-Design HZD Loop}

URDFs are generated automatically based on two parameters.

To do this it was necessary to make the inertial properties as functions of the link lengths. Make plots showing how the change together. 

\begin{algorithm}
\caption{HZD Co-Design Algorithm}\label{alg:co_design_hzd}
\begin{algorithmic}
\State {$D_t = [{t_{min}:\Delta_t:{t_{max}}}] \in \mathbb{R}^N$}
\State {$D_s = [{s_{min}:\Delta_s:{s_{max}}}] \in \mathbb{R}^M$}
\For{$n = 1$ to $N$}                    
    \For{$m = 1$ to $M$}                    
        \State {$\alpha_{t, 0} = D_{t}(i)$}
        \State {$\alpha_{s, 0} = D_{s}(j)$}
        \State {$k = 0$}
        \While{$|\alpha_{t, k} - \alpha_{t, k-1}| + |\alpha_{s, k} - \alpha_{s, k-1}| > \Delta$} 
            \State {$k = k + 1$}
            \State {$model = GenerateModel(\alpha_{t, k-1}, \alpha_{s, k-1})$}
            \State {$[\alpha_{t, k}, \alpha_{s, k}] = Solve(NLP, model)$}
        \EndWhile
        \State {$\alpha^{i, j}_{t, final} = \alpha_{t, k}$}
        \State {$\alpha^{i, j}_{s, final} = \alpha_{s, k}$}
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

\blue{Merge with previous section}

\begin{table}
\caption{A table showing additional parameters added to the gait to shape it.}
\label{tab:gait_constraints}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Variable & Lower Limit & Upper Limit\\
\hline
Step Length & $0.15 [m]$ & $0.35 [m]$ \\
\hline
Step Duration & $0.6 [s]$ & $0.9 [s]$ \\
\hline
Thigh Length & $0.15 [m]$ & $0.35 [m]$ \\
\hline
Shin Length & $0.15 [m]$ & $0.35 [m]$ \\
\hline
\end{tabular}
\end{center}
\end{table}

In this section we analyze the results obtained after running the algorithm presented in \ref{sec:co_design_framework}. The algorithm was ran for 441 different initial conditions where the initial thigh and shin lengths were uniformly distributed in a 2D grid between the minimum and maximum values from Tab. \ref{tab:gait_constraints}. 

Fig. \ref{fig:convergence_of_lengths} visualizes how the link lengths converge very closely to the same values irrespective of their initial values. In Tab. \ref{tab:optimization_results} several of the key parameters from the optimization is presented. From the table it can be seen that the optimal thigh length of $0.25 m$ is slightly shorter than the optimal shin length of $0.26 m$. Both variables converged with a very high accuracy where the standard deviation (std) is below $1.5e-3$ for both.  

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/converged_lengths.eps}
    \caption{A figure how the link lengths and thigh lengths converge from their initial values when using Co-Design-HZD algorithm.}
    \label{fig:convergence_of_lengths}
\end{figure}

\begin{table}
\caption{A table showing the average of and mean for the converged gaits after running from 25 different initial link length combinations.}
\label{tab:optimization_results}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Parameter & Mean Limit & Std \\
\hline
Thigh Length & $0.2477 [m]$ & $0.7e-3 [m]$ \\
\hline
Shin Length & $0.2590 [m]$ & $1.5e-3 [m]$ \\
\hline
Step Length & $0.2936 [m]$ & $0.0261 [m]$ \\
\hline
Step Duration & $0.8570 [s]$ & $0.90296 [s]$ \\
\hline
Walking Speed & $0.3420 [m/s]$ & $0.0196 [m/s]$ \\
\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Computational Cost}

The entire optimization loop took approximately 20 hours to run, where the run time scales linearly, O(n) with the number of samples. For the experiment ran here we chose to use a large number of samples to demonstrate consistency of the method across a wide range of initial conditions. In general, when applying the method to a specific hybrid zero system, you could get away with a significantly lower number of samples. Figure xxx shows how the design variables converge very fast, even with only a few samples. 

The most time consuming part of each sample optimization is the generation of the mex files used in FROST. These account for about XXX percent of the time, so an optimization tool not using this is likely to be able to speed up the process significantly. The time to generate the mex files scales quadratically $O(n^2)$ with the number of DoFs, therefore it can be wise to remove irrelevant DoFs when performing the optimization loop.

% Talk about how reasonable the results are by comparing it to a human of similar diemsions. 

% Add point in the table on how many iterations that were necessary to get convergence in each case. Explain how the link lengths often converge very fast to their near final values and that the values do not change too much after updating the model, which makes sense as the inertial changes are not drastic. 




